H2O-SDF: Two-phase Learning for 3D Indoor Reconstruction using Object Surface Fields

Advanced techniques using Neural Radiance Fields (NeRF), Signed Distance Fields (SDF), and Occupancy Fields have recently emerged as solutions for 3D indoor scene reconstruction. We introduce a novel two-phase learning approach, H2O-SDF, that discriminates between object and non-object regions within indoor environments. This method achieves a nuanced balance, carefully preserving the geometric integrity of room layouts while also capturing intricate surface details of specific objects. A cornerstone of our two-phase learning framework is the introduction of the Object Surface Field (OSF), a novel concept designed to mitigate the persistent vanishing gradient problem that has previously hindered the capture of high-frequency details in other methods. Our proposed approach is validated through several experiments that include ablation studies.

==> Figure/tex/Ablation_study.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{Figure/pdf/Exp_ablation.pdf}
%     \caption{Visualization Results of the ablation study.}
%     \label{fig:ablation}
% \end{figure}

% \setlength\intextsep{0pt}
% \begin{figure}[t]
%     \centering
%     \begin{tikzpicture}
%         \node at (0,0) {\includegraphics[width=\textwidth]{Figure/pdf/Exp_ablation.pdf}};
%         \node[font=\small] at (-5.85,-1.25) {NeuS};
%         \node[font=\small] at (-3.5,-1.25)  {Model A};
%         \node[font=\small] at (-1.15,-1.25) {Model B};
%         \node[font=\small] at (1.24,-1.25)  {Model C};
%         \node[font=\small] at (3.5,-1.25)   {$\text{H}_2\text{O-SDF}$};
%         \node[font=\small] at (5.9,-1.25)   {Ground Truth};
%     \end{tikzpicture}
%     \caption{Visualization Results of our Ablation Study}
%     \label{fig:ablation}
% \end{figure}


%ver1
\setlength\intextsep{0pt}
\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        \node at (0,0) {\includegraphics[width=\textwidth]{Figure/pdf/Exp_ablation.pdf}};
        \node[font=\small] at (-5.85,-1.25) {NeuS};
        \node[font=\small] at (-3.5,-1.25) {Model A};
        \node[font=\small] at (-1.15,-1.25) {Model B};
        \node[font=\small] at (1.24,-1.25) {$\text{H}_2\text{O-SDF \scriptsize{w/o OGS}}$};
        \node[font=\small] at (3.5,-1.25) {$\text{H}_2\text{O-SDF}$ };
        \node[font=\small] at (5.9,-1.25) {Ground Truth};
    \end{tikzpicture}
    \caption{Visualization Results of our Ablation Study.}
    \label{fig:ablation}
\end{figure}


    

==> Figure/tex/Method_point_sampling.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{Figure/pdf/samping_figure.PNG}
    \caption{Comparison Point Sampling Scheme with the Previous Method and Our Method.}
    \label{fig:method_point}
\end{figure}


==> Figure/tex/supple/Supple_nvs.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{Figure/pdf/supple/supple_nvs.pdf}
    \caption{Novel view synthesis results.}
    \label{fig:supple_nvs}
\end{figure}

==> Figure/tex/supple/supple_replica.tex <==
% \begin{figure}
% % \includegraphics[trim=6cm 3.5cm 7cm 4.1cm, clip, width=\textwidth]{Figure/pdf/supple/supple_replica.pdf}

% \begin{minipage}{\textwidth}
%     \centering
%     \includegraphics[trim=6cm 2cm 6cm 2cm, clip, width=\textwidth]{Figure/pdf/supple/replica_result_birdview_v2.pdf}
%     \fontsize{10}{1}\selectfont
%     \vspace{-5pt}
%     \hspace{2.3cm} NeuRIS \hspace{3cm} Ours \hspace{3.3cm} Reference
% \end{minipage}
% \vspace{5pt}
% \caption{ \textbf{Evaluation on Replica dataset.}
% }\label{fig:supple_replica}
% % \vspace{-5pt}
% \end{figure}


\begin{figure}[h]
    % \centering
    \begin{tikzpicture}
        \node at (0,0) {\includegraphics[trim=6cm 2cm 6cm 2cm, clip, width=\textwidth]{Figure/pdf/supple/replica_result_birdview_v2.pdf}};
        \node[font=\large] at (-4,0.25) {(a)};
        \node[font=\large] at (0.5,0.25) {(b)};
        \node[font=\large] at (5,0.25) {(c)};
        \node[font=\large] at (-4,-4.7) {(d)};
        \node[font=\large] at (0.5,-4.7) {(e)};
        \node[font=\large] at (5,-4.7) {(f)};
    \end{tikzpicture}
    \caption{Qualitative Visualization on Replica Dataset}
    \label{fig:supple_replica}
\end{figure}

==> Table/Ablation_study.tex <==
% \vspace{-2mm}
% \begin{table}[ht]
% \centering
% \caption{Ablation Study on 13 Scene ScanNet }
% \scriptsize
% \begin{tabular}{M{2.5cm}M{1.2cm}M{1.2cm}M{1.2cm}M{1.2cm}M{1.2cm}}
% \Xhline{3\arrayrulewidth}
% \\ [-0.9em]
% Methods & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ 
% \\ [0.1em]
% \Xhline{0.3\arrayrulewidth}
% %Method& Acc$\downarrow$& Comp$\downarrow$& Prec$\uparrow$& Recall$\uparrow$& F-score$\uparrow$\\ 
% \\ [-0.9em]
% NeuS          & 0.131      & 0.12      & 0.376      & 0.33     & 0.35         
% \\ [0.1em]
% \\ [-0.9em]
% Model A       & 0.041      & 0.043     & 0.786      & 0.738    & 0.76        
% \\ [0.1em]
% \\ [-0.9em]
% Model B       & 0.042      & 0.042     & 0.794      & 0.748   &0.77 
% \\ [0.1em]
% \\ [-0.9em]
% Model C       & 0.04      & 0.041      & 0.82      & 0.757        & 0.785
% \\ [0.1em]
% \Xhline{0.3\arrayrulewidth}
% \\ [-0.9em]
% \textbf{Ours} & \textbf{0.038} & \textbf{0.04} & \textbf{0.823} & \textbf{0.768} & \textbf{0.794} 
% \\ [0.1em]
% \Xhline{2\arrayrulewidth}
% \end{tabular}
% \label{tab:ablation}
% \end{table}

\setlength\intextsep{0pt}
\vspace{-2mm}
\begin{table}[t]
\centering

\scriptsize
\begin{tabular}{M{2.0cm} | M{0.5cm} M{0.5cm} M{0.5cm} M{0.5cm} M{0.6cm} | M{0.8cm}M{0.8cm}M{0.8cm}M{0.8cm}M{1.0cm}}
\Xhline{3\arrayrulewidth}
\\ [-0.9em]
Method &NeuS &Normal &HSL &OSL &OGS &Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ 
\\ [0.1em]
\Xhline{0.3\arrayrulewidth}
%Method& Acc$\downarrow$& Comp$\downarrow$& Prec$\uparrow$& Recall$\uparrow$& F-score$\uparrow$\\ 
\\ [-0.9em]
NeuS &\checkmark &- &- &- &- &0.132      & 0.114      & 0.376      & 0.334     & 0.353         
\\ [0.1em]
\\ [-0.9em]
Model A &\checkmark &\checkmark &- &- &-       & 0.040      & 0.042     & 0.794      & 0.742    & 0.766        
\\ [0.1em]
\\ [-0.9em]
Model B &\checkmark &\checkmark &\checkmark &- &-        & 0.041      & 0.041     & 0.802      & 0.751   &0.776 
\\ [0.1em]
\Xhline{0.3\arrayrulewidth}
\\ [-0.9em]
$\text{H}_2\text{O-SDF w/o OGS}$  &\checkmark &\checkmark &\checkmark &\checkmark &-      & 0.039      & 0.041      & 0.817      & 0.762        & 0.787
\\ [0.1em]
\\ [-0.9em]
$\text{H}_2\text{O-SDF}$ &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark     & \textbf{0.037} & \textbf{0.039} & \textbf{0.830} & \textbf{0.773} & \textbf{0.800} 
\\ [0.1em]
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{Quantitative Results on the Ablation Study of 12 scene ScanNet }
\label{tab:ablation_ver2}
\end{table}

==> Table/Quantitative_3D.tex <==
%Ver1
\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{M{2.5cm}| M{1.0cm}M{1.0cm}M{1.0cm}M{1.0cm}M{1.5cm}}
\Xhline{3\arrayrulewidth}
\\ [-0.5em]

Methods & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ 
\\ [0.5em]
\Xhline{0.3\arrayrulewidth}
%Method& Acc$\downarrow$& Comp$\downarrow$& Prec$\uparrow$& Recall$\uparrow$& F-score$\uparrow$\\ 
\\ [-0.8em]
COLMAP        & 0.047      & 0.235      & 0.711      & 0.441        & 0.537       
\\ [0.2em]
\\ [-1.0em]
ACMP          & 0.118      & 0.081      & 0.531      & 0.581        & 0.555         
\\ [0.2em]
\Xhline{0.3\arrayrulewidth}
\\ [-1.0em]
NeRF          & 0.735      & 0.177      & 0.131      & 0.290         & 0.176         
\\ [0.2em]
\\ [-1.0em]
VolSDF        & 0.414      & 0.120       & 0.321      & 0.394        & 0.346        
\\ [0.2em]
\\ [-1.0em]
NeuS          & 0.179      & 0.208      & 0.313      & 0.275        & 0.291         
\\ [0.2em]
\Xhline{0.3\arrayrulewidth}
\\ [-1.0em]
ManhattanSDF& 0.053      & 0.056      & 0.715      & 0.664        & 0.688        
\\ [0.2em]
\\ [-1.0em]
NeuRIS        & 0.052      & 0.050       & 0.713      & 0.677        & 0.690 
\\ [0.2em]
\\ [-1.0em]
MonoSDF       & 0.035      & 0.048      & 0.799      & 0.681        & 0.733
\\ [0.2em]
\\ [-1.0em]
HelixSurf     & 0.038      & 0.044      & 0.786      & 0.727        & 0.755         
\\ [0.2em]
\Xhline{0.3\arrayrulewidth}
\\ [-1.0em]
$\text{H}_2\text{O-SDF}$ w/o OGS     & 0.034       & 0.0382     & 0.821      & 0.761        & 0.789
\\ [0.2em]
\textbf{$\text{H}_2\text{O-SDF}$} & \textbf{0.032} & \textbf{0.0373} & \textbf{0.834} & \textbf{0.769} & \textbf{0.799} 
\\ [0.2em]
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{\textbf{Quantitative Comparison on ScanNet} We compare $\text{H}_2\text{O-SDF}$ against other previous state-of-the-art methods. OGS indicates the object surface field guided sampling.} 
\label{tab:3d_quantitative}
\end{table}




% \begin{tabular}{M{1.0cm}M{0.65cm}M{0.65cm}M{0.65cm}M{0.65cm}M{0.65cm}}
% \Xhline{3\arrayrulewidth}
% \\ [-0.5em]
% Methods & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ 
% \\ [0.5em]
% \Xhline{0.3\arrayrulewidth}
% %Method& Acc$\downarrow$& Comp$\downarrow$& Prec$\uparrow$& Recall$\uparrow$& F-score$\uparrow$\\ 
% \\ [-0.8em]
% COLMAP        & 0.047      & 0.235      & 0.711      & 0.441        & 0.537       
% \\ [0.2em]
% \\ [-0.8em]
% ACMP          & 0.118      & 0.081      & 0.531      & 0.581        & 0.555         
% \\ [0.2em]
% \Xhline{0.3\arrayrulewidth}
% \\ [-0.8em]
% NeRF          & 0.735      & 0.177      & 0.131      & 0.290         & 0.176         
% \\ [0.2em]
% \\ [-0.8em]
% VolSDF        & 0.414      & 0.120       & 0.321      & 0.394        & 0.346        
% \\ [0.2em]
% \\ [-0.8em]
% NeuS          & 0.179      & 0.208      & 0.313      & 0.275        & 0.291         
% \\ [0.2em]
% \Xhline{0.3\arrayrulewidth}
% \\ [-0.8em]
% Manhattan & 0.053      & 0.056      & 0.715      & 0.664        & 0.688        
% \\ [0.2em]
% \\ [-0.8em]
% NeuRIS        & 0.052      & 0.050       & 0.713      & 0.677        & 0.690 
% \\ [0.2em]
% \\ [-0.8em]
% MonoSDF       & 0.035      & 0.048      & 0.799      & 0.681        & 0.733
% \\ [0.2em]
% \\ [-0.8em]
% HelixSurf     & 0.038      & 0.044      & 0.786      & 0.727        & 0.755         
% \\ [0.2em]
% \Xhline{0.3\arrayrulewidth}
% \\ [-0.8em]
% \textbf{Ours} & \textbf{0.032} & \textbf{0.0373} & \textbf{0.834} & \textbf{0.769} & \textbf{0.799} 
% \\ [0.2em]
% \Xhline{2\arrayrulewidth}
% \end{tabular}
% \label{tab:3d_quantitative}


==> Table/Sup_quantitative_normal_v1.tex <==
\begin{table}[ht]
\centering
\scriptsize

\begin{tabular}{M{2.5cm}| M{1.0cm}M{1.0cm}M{1.0cm} M{1.0cm} M{1.0cm} M{1.0cm}}
\Xhline{3\arrayrulewidth}
\\ [-0.5em]
Methods & Mean$\downarrow$ & Median$\downarrow$ & RMSE$\downarrow$ & $11.25\,^{\circ}$$\uparrow$ &$22.5\,^{\circ}$$\uparrow$ & $30\,^{\circ}$$\uparrow$
\\ [0.5em]
\Xhline{0.3\arrayrulewidth}
\\ [-0.8em]
TiltedSN     &14.8    &7.95    &23.32  &64.01  &79.95 &85.34     
\\ [0.2em]
\\ [-0.8em]
NeuRIS       &15.21   &8.77    &23.19  &61.46  &79.76 &85.42 
\\ [0.2em]
\Xhline{0.3\arrayrulewidth}
\\ [-0.8em]
$\text{H}_2\text{O-SDF w/o OGS}$ &14.59 &7.48 &22.77  &62.78 &79.77 &85.60 \\
\\ [-0.8em]
\textbf{$\text{H}_2\text{O-SDF}$} & \textbf{13.48} & \textbf{6.96} & \textbf{21.73} & \textbf{66.94} & \textbf{81.82} &\textbf{86.90}
\\ [0.2em]
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{Quantitative normal comparisons over 13 scene ScanNet }
\label{tab:normal_quantitative}
\end{table}

% \begin{tabular}{M{1.3cm} M{0.65cm}M{0.65cm}M{0.65cm} M{0.65cm} M{0.65cm} M{0.65cm}}
% \Xhline{3\arrayrulewidth}
% \\ [-0.5em]
% Methods & Mean$\downarrow$ & Median$\downarrow$ & RMSE$\downarrow$ & $11.25\,^{\circ}$$\uparrow$ &$22.5\,^{\circ}$$\uparrow$ & $30\,^{\circ}$ $\uparrow$
% \\ [0.5em]
% \Xhline{0.3\arrayrulewidth}
% \\ [-0.8em]
% ManhattanSDF &19.14   &10.82   &29.43  &52.86  &74.4  &80.96   
% \\ [0.2em]
% \\ [-0.8em]
% HelixSurf    &19.3    &11.92   &28.87  &47.19  &74.43 &82.16         
% \\ [0.2em]
% \\ [-0.8em]
% TiltedSN     &14.8    &7.95    &23.32  &64.01  &79.95 &85.34     
% \\ [0.2em]
% \\ [-0.8em]
% NeuRIS       &15.21   &8.77    &23.19  &61.46  &79.76 &85.42 
% \\ [0.2em]

% \Xhline{0.3\arrayrulewidth}
% \\ [-0.8em]
% \textbf{Ours} & \textbf{13.48} & \textbf{6.96} & \textbf{21.73} & \textbf{66.94} & \textbf{81.82} &\textbf{86.9}
% \\ [0.2em]
% \Xhline{2\arrayrulewidth}
% \end{tabular}
% \label{tab:normal_quantitative}



% \\ [-0.8em]
% ManhattanSDF &19.14   &10.82   &29.43  &52.86  &74.4  &80.96   
% \\ [0.2em]
% \\ [-0.8em]
% HelixSurf    &19.3    &11.92   &28.87  &47.19  &74.43 &82.16         
% \\ [0.2em]

==> Table/Supple_3D_ver2.tex <==
\newcolumntype{g}{>{\columncolor{Gray}}c}
\begin{table}[htbp]
  \scriptsize
  \centering
  \label{tbl:wasss}
  \caption{Quantitative comparisons of individual scenes on ScanNet.}
  \begin{tabular}{|c|c c c c c|}
    \hline
    \multirow{2}{*}{Method} &\multicolumn{5}{c|}{Scene0002\_00} \\
     \cline{2-11}
     & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ \\\hline
    ManhattanSDF & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    NeuRIS      &0.032	&0.046	&0.85	&0.726	&0.783 & 0.046 & 0.048 & 0.77 & 0.748 & 0.759 \\
    \rowcolor{Gray}
    Ours        &0.029	&0.046	&0.873	&0.74 &0.801 &0.06 &0.046 &0.713 &0.731 &0.722 \\
    \hline
    &\multicolumn{5}{c|}{Scene0009\_00}
    & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ \\\hline
    ManhattanSDF & 0 & 0 & 0 & 0 & 0 \\
    NeuRIS      &0.046 & 0.048 & 0.77 & 0.748 & 0.759 \\
    \rowcolor{Gray}
    Ours        &0.06 &0.046 &0.713 &0.731 &0.722 \\
    \hline
    \multirow{2}{*}{Method} &\multicolumn{5}{c|}{Scene0012\_00} \\
     \cline{2-11}
     & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ \\\hline
    ManhattanSDF & 0 & 0 & 0 & 0 & 0\\
    NeuRIS       &0.025	&0.029	&0.92 &0.867 &0.893  \\
    \rowcolor{Gray}
    Ours         &0.024 &0.028 &0.93 &0.875 &0.901  \\

    \hline
     \multirow{2}{*}{Method} &\multicolumn{5}{c|}{Scene0050\_00} \\
     \cline{2-11}
     & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ \\\hline
    ManhattanSDF & 0 & 0 & 0 & 0 & 0  \\
    NeuRIS       &0.043	&0.042	&0.774	&0.732	&0.752 \\
    \rowcolor{Gray}
    Ours          &0.03 &0.036 &0.856 &0.784	&0.818 \\
    \hline
    \hline
    \multirow{2}{*}{Method} &\multicolumn{5}{c|}{Scene0084\_00} &\multicolumn{5}{c|}{Scene0114\_02} \\
     \cline{2-11}
     & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ \\\hline
    ManhattanSDF & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    NeuRIS      &0.052	&0.047	&0.695	&0.695	&0.679 &0.063	&0.06	&0.635	&0.6	&0.617 \\
    \rowcolor{Gray}
    Ours       &0.027	&0.029	&0.893	&0.855	&0.874 &0.063 &0.057 &0.704	&0.682 &0.693 \\
    \hline
    \hline
    \multirow{2}{*}{Method} &\multicolumn{5}{c|}{Scene0279\_00} &\multicolumn{5}{c|}{Scene0580\_00} \\
     \cline{2-11}
     & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ \\\hline
    ManhattanSDF & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    NeuRIS      &0.066	&0.057	&0.685	&0.651	&0.668 &0.065	&0.052	&0.671	&0.667	&0.669 \\
    \rowcolor{Gray}
    Ours       &0.043	&0.042	&0.789	&0.734	&0.76 &0.031 &0.034	&0.863 &0.827 &0.845 \\
    \hline
    \hline
    \multirow{2}{*}{Method} &\multicolumn{5}{c|}{Scene0603\_00} &\multicolumn{5}{c|}{Scene0616\_00} \\
     \cline{2-11}
     & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ \\\hline
    ManhattanSDF & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    NeuRIS      &0.039	&0.049	&0.8	&0.693	&0.743 &0.048	&0.057	&0.712	&0.614	&0.659 \\
    \rowcolor{Gray}
    Ours       &0.043	&0.049	&0.784	&0.689	&0.734 &0.04	&0.051	&0.73	&0.615	&0.667 \\
    \hline
    \hline
    \multirow{2}{*}{Method} &\multicolumn{5}{c|}{Scene0617\_00} &\multicolumn{5}{c|}{Scene0625\_00} \\
     \cline{2-11}
     & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ \\\hline
    ManhattanSDF & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
    NeuRIS      &0.067	&0.057	&0.731	&0.695	&0.713 &0.027	&0.025	&0.885	&0.882	&0.883 \\
    \rowcolor{Gray}
    Ours       &0.049	&0.047	&0.771	&0.726	&0.748  &0.019	&0.017	&0.975	&0.986	&0.981 \\
    \hline
    \hline
    \multirow{2}{*}{Method} &\multicolumn{5}{c|}{Scene0721\_00} \\
    \cline{2-6}
     & Acc$\downarrow$ & Comp$\downarrow$ & Prec$\uparrow$ & Recall$\uparrow$  & F-score$\uparrow$ \\\cline{1-6}
     ManhattanSDF & 0 & 0 & 0 & 0 & 0 \\
     NeuRIS      &0.043	&0.041	&0.785	&0.734	&0.759 \\
     \rowcolor{Gray}
     Ours       &0.043	&0.039	&0.8	&0.765	&0.786 \\
     \cline{1-6}
  \end{tabular}
  
  \label{tbl:wasss}
\end{table}

==> Table/Supple_7scenes.tex <==
%% Table for common comments.
% 7-scenes
\begin{table}[h!]
\centering
\small
\begin{tabular}{c|cccccc}
\Xhline{3\arrayrulewidth}
\\ [-0.8em]
Model & Accu.$\downarrow$ & Comp.$\downarrow$ & Prec.$\uparrow$ & Recall$\uparrow$ & F-score$\uparrow$ \\ 
\hline
\\ [-0.8em]
ManhattanSDF & \textbf{0.112} & 0.132 & 0.351 & 0.326 & 0.336 \\
\\ [-0.9em]
NeuRIS & 0.133 & 0.132 & 0.405 & 0.424 & 0.410 \\
\\ [-0.9em]
MonoSDF &0.158	&0.328	&0.286	&0.262	&0.301\\
\\ [-0.9em]
\hline
\\ [-0.9em]
$\text{H}_2\text{O-SDF}$ & 0.128 & \textbf{0.129} & \textbf{0.416} & \textbf{0.469} & \textbf{0.447}
\\ 
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Comparison results for 7-Scenes}
\label{tab:sup_7scenes}
\end{table}

% \begin{table}[h]
% \centering
% \small
% \begin{tabular}{M{3.0cm}| M{1.1cm} M{1.1cm} M{1.1cm} M{1.1cm} M{1.1cm}}
% \Xhline{3\arrayrulewidth}
% \\ [-0.5em]
% Methods & Accu.$\downarrow$ & Comp.$\downarrow$ & Prec.$\uparrow$ & Recall$\uparrow$ & F-score$\uparrow$
% \\ [0.5em]
% \Xhline{0.3\arrayrulewidth}
% \\ [-0.8em]
% ManhattanSDF & 0.112 & 0.132 & 0.351 & 0.326 & 0.336 \\
% \\ [0.2em]
% \\ [-0.8em]
% NeuRIS & 0.133 & 0.132 & 0.405 & 0.424 & 0.410 \\
% \\ [0.2em]
% \\ [-0.8em]
% MonoSDF & 0.112 & 0.132 & 0.351 & 0.326 & 0.336 \\
% \\ [0.2em]

% \Xhline{0.3\arrayrulewidth}
% \\ [-0.8em]
% \textbf{$\text{H}_2\text{O-SDF}$} & \textbf{0.128} & \textbf{0.129} & \textbf{0.416} & \textbf{0.469} & \textbf{0.447} 
% \\ [0.2em]
% \Xhline{2\arrayrulewidth}
% \end{tabular}
% \caption{Comparison results for 7-Scenes}
% \label{tab:7scenes}
% \end{table}

==> Table/Supple_general_exp_ver2.tex <==
\begin{table}[b]
\centering
\scriptsize

\resizebox{\textwidth}{!}{
\subfloat[Evaluation Metrics for 3D Reconstruction Result]{
        \begin{tabular}{M{1.5cm} M{5.0cm}}
            \Xhline{3\arrayrulewidth}
            \\ [-0.5em]
            Methods & Definition
            \\ [0.5em]
            \Xhline{0.3\arrayrulewidth}
            \\ [-0.2em]
            Accuracy        & $\mathrm{mean}_{\mathbf{p}\in \mathcal{\mathcal{P}}}(\mathrm{min}_{\mathbf{p}^{*} \in \mathcal{P}^{*}} \left\| \mathbf{p} - \mathbf{p}^{*} \right\| )$
            \\ [0.5em]
            \\ [-0.5em]
            Completeness    & $\mathrm{mean}_{\mathbf{p}^*\in \mathcal{P}^*}(\mathrm{min}_{\mathbf{p} \in \mathcal{P}} \left\| \mathbf{p} - \mathbf{p}^{*} \right\| )$
            \\ [0.5em]
            \\ [-0.5em]
            Precision       & $\mathrm{mean}_{\mathbf{p}\in \mathcal{P}}(\mathrm{min}_{\mathbf{p}^* \in \mathcal{P}^*} \left\| \mathbf{p} - \mathbf{p}^{*} \right\| < 0.05)$
            \\ [0.5em]
            \\ [-0.5em]
            Recall          & $\mathrm{mean}_{\mathbf{p}^*\in \mathcal{P}^*}(\mathrm{min}_{\mathbf{p} \in \mathcal{P}} \left\| \mathbf{p} - \mathbf{p}^{*} \right\| < 0.05)$
            \\ [0.5em]
            \\ [-0.5em]
            F-score         & $\frac{2\times \mathrm{Precision} \times \mathrm{Recall}}{\mathrm{Precision} + \mathrm{Recall}}$
            \\ [0.5em]
            \\ [-0.2em]            
            \Xhline{2\arrayrulewidth}
            \label{sub:3d_metrics}
        \end{tabular}}
\subfloat[Evaluation Metrics for Rendered Normal Result]{
        \begin{tabular}{M{1.5cm} M{5.0cm}}
            \Xhline{3\arrayrulewidth}
            \\ [-0.5em]
            Methods & Definition
            \\ [0.5em]
            \Xhline{0.3\arrayrulewidth}
            \\ [-0.6em]
            Mean                        & $\frac{1}{N}\sum \mathrm{cos}^{-1}\left[ \frac{ \left| \mathbf{n} \cdot \mathbf{n}^* \right| }{\left|\mathbf{n}\right| \left|\mathbf{n}^* \right| } \right] $
            \\ [0.5em]
            \\ [-0.5em]
            Median                      & $\mathrm{median} \left\{ \mathrm{cos}^{-1} \left[ \frac{ \left| \mathbf{n} \cdot \mathbf{n}^* \right| }{\left|\mathbf{n}\right| \left|\mathbf{n}^* \right| } \right]\right\}$
            \\ [0.5em]
            \\ [-0.5em]
            RMSE                        & $\sqrt{\frac{1}{N}\sum (\mathrm{cos}^{-1}\left[ \frac{ \left| \mathbf{n} \cdot \mathbf{n}^* \right| }{\left|\mathbf{n}\right| \left|\mathbf{n}^* \right| } \right])^2}$
            \\ [0.5em]
            \\ [-0.5em]
            $\mathbf{deg}^{\circ}$      & $\frac{1}{N}\{ \mathbf{n}, \mathbf{n}^* : cos^{-1}\left[ \frac{ \left| \mathbf{n} \cdot \mathbf{n}^* \right| }{\left|\mathbf{n}\right| \left|\mathbf{n}^* \right| } \right] < \mathbf{deg}^{\circ} \}$
            \\ [0.5em]
            \\ [-0.5em]
            \Xhline{2\arrayrulewidth}
            \label{sub:normal_metrics}
        \end{tabular}
        }}
\caption{Evaluation Metrics}
\label{tab:eval_metric_3d}
\end{table}

==> Table/Supple_replica.tex <==
\begin{table}[h!]
\centering
\small
\begin{tabular}{c|cccccc}
\Xhline{3\arrayrulewidth}
\\ [-0.8em]
Model & Accu.$\downarrow$ & Comp.$\downarrow$ & Prec.$\uparrow$ & Recall$\uparrow$ & F-score$\uparrow$ \\ 
\hline
\\ [-0.8em]
ManhattanSDF & 0.131 & 0.417 & 0.644 & 0.407 & 0.492 \\
\\ [-0.8em]
NeuRIS & 0.023 & 0.027 & 0.921 & 0.898 & 0.909 \\
\\ [-0.8em]
MonoSDF & 0.020 & 0.017 & 0.951 & 0.923 & 0.934 \\
\\ [-0.8em]
\hline
\\ [-0.8em]
$\text{H}_2\text{O-SDF}$ & \textbf{0.016} & \textbf{0.025} & \textbf{0.983} & \textbf{0.935} & \textbf{0.957} \\ 
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Comparison results for Replica}
\label{tab:sup_replica}
\end{table}
